Decoupled Access-Execute enabled DVFS for tinyML deployments on STM32 microcontrollers

Over the last years the rapid growth Machine Learning (ML) inference applications deployed on the Edge is rapidly increasing. Recent Internet of Things (IoT) devices and microcontrollers (MCUs), become more and more mainstream in everyday activities. In this work we focus on the family of STM32 MCUs. We propose a novel methodology for CNN deployment on the STM32 family, focusing on power optimization through effective clocking exploration and configuration and decoupled access-execute convolution kernel execution. Our approach is enhanced with optimization of the power consumption through Dynamic Voltage and Frequency Scaling (DVFS) under various latency constraints, composing an NP-complete optimization problem. We compare our approach against the state-of-the-art TinyEngine inference engine, as well as TinyEngine coupled with power-saving modes of the STM32 MCUs, indicating that we can achieve up to 25.2% less energy consumption for varying QoS levels.

==> figures/methodology_twocol <==
<mxfile host="app.diagrams.net" modified="2023-09-13T14:14:37.161Z" agent="Mozilla/5.0 (X11; Linux x86_64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/91.0.4472.114 Safari/537.36" etag="ysuamHEnoGBLx5MzGOy1" version="21.7.5" type="device">
  <diagram name="Page-1" id="XB__WySE0HvbIRqd7pLn">
    <mxGraphModel dx="524" dy="256" grid="1" gridSize="10" guides="1" tooltips="1" connect="1" arrows="1" fold="1" page="1" pageScale="1" pageWidth="827" pageHeight="1169" math="1" shadow="0">
      <root>
        <mxCell id="0" />
        <mxCell id="1" parent="0" />
        <mxCell id="oelAyTeBvST4LJL2yoes-25" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#f5f5f5;dashed=1;strokeWidth=0.6;fontColor=#333333;strokeColor=#666666;" vertex="1" parent="1">
          <mxGeometry x="646" y="168.93" width="54" height="97" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-4" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.polygon;polyCoords=[[0.06,0],[0.94,0],[1,0.1],[1,0.91],[0.94,1],[0.05,1],[0,0.91],[0,0.1]];polyline=0;fillColor=none;strokeWidth=0.6;dashed=1;" parent="1" vertex="1">
          <mxGeometry x="356" y="99" width="199" height="170" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-80" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.polygon;polyCoords=[[0.06,0],[0.94,0],[1,0.1],[1,0.91],[0.94,1],[0.05,1],[0,0.91],[0,0.1]];polyline=0;fillColor=none;strokeWidth=0.6;dashed=1;" parent="1" vertex="1">
          <mxGeometry x="126" y="100" width="225" height="170" as="geometry" />
        </mxCell>
        <mxCell id="xOS6cA8aV1tglOhgtO3--1" value="Pre-trained &lt;br style=&quot;font-size: 12px;&quot;&gt;(optimized) CNN model" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Latin Modern Roman;fontSize=12;fontStyle=0" parent="1" vertex="1">
          <mxGeometry x="19" y="69" width="90" height="46" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-81" value="" style="endArrow=classic;html=1;rounded=0;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=0.5;entryY=0;entryDx=0;entryDy=0;strokeWidth=0.6;" parent="1" source="vccc8psbofyykT3IaAuy-69" target="vccc8psbofyykT3IaAuy-82" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="410" y="150" as="sourcePoint" />
            <mxPoint x="460" y="100" as="targetPoint" />
            <Array as="points">
              <mxPoint x="120" y="213" />
              <mxPoint x="120" y="184" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-82" value="Layer Selection" style="rounded=0;whiteSpace=wrap;html=1;rotation=-90;fillColor=#f5f5f5;fontColor=#000000;strokeColor=#666666;fontFamily=Latin Modern Roman;" parent="1" vertex="1">
          <mxGeometry x="91.5" y="174.5" width="110" height="19" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-84" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#94F7B5;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="1" vertex="1">
          <mxGeometry x="180" y="142.5" width="30" height="27" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-85" value="" style="endArrow=classic;html=1;rounded=0;exitX=0.75;exitY=1;exitDx=0;exitDy=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;strokeWidth=0.6;" parent="1" source="vccc8psbofyykT3IaAuy-82" target="vccc8psbofyykT3IaAuy-84" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="210" y="190" as="sourcePoint" />
            <mxPoint x="260" y="140" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-86" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E8B3E4;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="1" vertex="1">
          <mxGeometry x="180" y="197.5" width="30" height="27" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-87" value="" style="endArrow=classic;html=1;rounded=0;exitX=0.25;exitY=1;exitDx=0;exitDy=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;strokeWidth=0.6;" parent="1" source="vccc8psbofyykT3IaAuy-82" target="vccc8psbofyykT3IaAuy-86" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="166" y="167" as="sourcePoint" />
            <mxPoint x="189" y="166" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-88" value="Pointwise&lt;br style=&quot;font-size: 10px;&quot;&gt;Conv. Layers" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Latin Modern Roman;fontSize=10;" parent="1" vertex="1">
          <mxGeometry x="159" y="111" width="80" height="30" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-89" value="Depthwise&lt;br style=&quot;font-size: 10px;&quot;&gt;Conv. Layers" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Latin Modern Roman;fontSize=10;" parent="1" vertex="1">
          <mxGeometry x="159" y="228" width="80" height="30" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-93" value="DAE-enabled Layers" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Latin Modern Roman;fontSize=10;" parent="1" vertex="1">
          <mxGeometry x="282.5" y="112.5" width="67" height="30" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-95" value="Access Execution Decoupling" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#f5f5f5;fontColor=#000000;strokeColor=#000000;rotation=-90;fontFamily=Latin Modern Roman;verticalAlign=middle;" parent="1" vertex="1">
          <mxGeometry x="201.63" y="160.07" width="113.12" height="47.87" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-96" value="" style="endArrow=classic;html=1;rounded=0;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=0.75;entryY=0;entryDx=0;entryDy=0;strokeWidth=0.6;" parent="1" source="vccc8psbofyykT3IaAuy-84" target="vccc8psbofyykT3IaAuy-95" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="310" y="190" as="sourcePoint" />
            <mxPoint x="360" y="140" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-97" value="" style="endArrow=classic;html=1;rounded=0;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=0.265;entryY=0.008;entryDx=0;entryDy=0;entryPerimeter=0;strokeWidth=0.6;" parent="1" source="vccc8psbofyykT3IaAuy-86" target="vccc8psbofyykT3IaAuy-95" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="221" y="166" as="sourcePoint" />
            <mxPoint x="247" y="166" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-99" value="" style="endArrow=classic;html=1;rounded=0;exitX=0.739;exitY=1.021;exitDx=0;exitDy=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;strokeWidth=0.6;exitPerimeter=0;" parent="1" source="vccc8psbofyykT3IaAuy-95" target="vccc8psbofyykT3IaAuy-98" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="278" y="157" as="sourcePoint" />
            <mxPoint x="382" y="140" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-101" value="" style="endArrow=classic;html=1;rounded=0;exitX=0.263;exitY=0.997;exitDx=0;exitDy=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;strokeWidth=0.6;exitPerimeter=0;" parent="1" source="vccc8psbofyykT3IaAuy-95" target="vccc8psbofyykT3IaAuy-100" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="278" y="211" as="sourcePoint" />
            <mxPoint x="311" y="166" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-104" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#94F7B5;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="1" vertex="1">
          <mxGeometry x="184" y="146" width="30" height="27" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-105" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E8B3E4;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="1" vertex="1">
          <mxGeometry x="184" y="201" width="30" height="27" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-107" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="298" y="139" width="38" height="36" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-98" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#94F7B5;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="vccc8psbofyykT3IaAuy-107" vertex="1">
          <mxGeometry x="4" y="4.5" width="30" height="27" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-108" value="" style="group" parent="vccc8psbofyykT3IaAuy-107" vertex="1" connectable="0">
          <mxGeometry x="4" y="4.5" width="34" height="31.5" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-109" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#94F7B5;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="vccc8psbofyykT3IaAuy-108" vertex="1">
          <mxGeometry x="4" y="4.5" width="30" height="27" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-111" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="298" y="193" width="45" height="36" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-100" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E8B3E4;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="vccc8psbofyykT3IaAuy-111" vertex="1">
          <mxGeometry x="4" y="4.5" width="30" height="27" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-112" value="" style="group" parent="vccc8psbofyykT3IaAuy-111" vertex="1" connectable="0">
          <mxGeometry x="4" y="4.5" width="41" height="31.5" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-113" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E8B3E4;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="vccc8psbofyykT3IaAuy-112" vertex="1">
          <mxGeometry x="4" y="4.5" width="30" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-237" value="" style="group" parent="vccc8psbofyykT3IaAuy-112" vertex="1" connectable="0">
          <mxGeometry x="17" y="4.5" width="24" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-238" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#28D4D4;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-237" vertex="1">
          <mxGeometry width="13" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-239" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-237" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="3" as="sourcePoint" />
            <mxPoint as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-240" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-237" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="6" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-241" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-237" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="9" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-242" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-237" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="12" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-243" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-237" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="15" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-244" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-237" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="18" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-245" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-237" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="21" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-246" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-237" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="24" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-247" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-237" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="27" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-2" value="&lt;font face=&quot;Latin Modern Roman&quot;&gt;&lt;b&gt;Step 1. Access Execution Decoupling (Sec. IIIA)&lt;/b&gt;&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#f5f5f5;fontColor=#000000;strokeColor=default;strokeWidth=0.6;shadow=1;" parent="1" vertex="1">
          <mxGeometry x="137" y="74" width="203" height="30" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-5" value="&lt;font face=&quot;Latin Modern Roman&quot;&gt;&lt;b&gt;Step 2. Frequency &amp;amp; Decoupling &lt;br&gt;Granularity DSE (Sec. IIIB)&lt;/b&gt;&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#f5f5f5;fontColor=#000000;strokeColor=default;strokeWidth=0.6;shadow=1;" parent="1" vertex="1">
          <mxGeometry x="356" y="74" width="200" height="30" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-7" value="1A" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fillColor=#000000;fontColor=#FFFFFF;fontFamily=Latin Modern Roman;fontSize=10;fontStyle=1" parent="1" vertex="1">
          <mxGeometry x="137.5" y="229" width="18" height="18" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-8" value="1B" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fillColor=#000000;fontColor=#FFFFFF;fontFamily=Latin Modern Roman;fontSize=10;fontStyle=1" parent="1" vertex="1">
          <mxGeometry x="270" y="229" width="18" height="18" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-12" value="" style="endArrow=classic;html=1;rounded=0;entryX=0;entryY=0.25;entryDx=0;entryDy=0;strokeWidth=0.6;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="337" y="162" as="sourcePoint" />
            <mxPoint x="366" y="181.24999999999977" as="targetPoint" />
            <Array as="points">
              <mxPoint x="345" y="162" />
              <mxPoint x="345" y="181" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-25" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="14" y="157" width="96" height="115" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-69" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#f5f5f5;dashed=1;strokeWidth=0.6;fontColor=#333333;strokeColor=#666666;" parent="T58t_aunDJeNxnw9ZxXW-25" vertex="1">
          <mxGeometry width="96" height="112" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-67" value="&lt;font style=&quot;font-size: 11px;&quot;&gt;3x3 dw-conv2d&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E8B3E4;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="T58t_aunDJeNxnw9ZxXW-25" vertex="1">
          <mxGeometry x="5" y="35" width="86" height="14" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-68" value="&lt;b&gt;...&lt;/b&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;rotation=90;" parent="T58t_aunDJeNxnw9ZxXW-25" vertex="1">
          <mxGeometry x="41" width="20" height="20" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-71" value="&lt;font style=&quot;font-size: 11px;&quot;&gt;3x3 dw-conv2d&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E8B3E4;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="T58t_aunDJeNxnw9ZxXW-25" vertex="1">
          <mxGeometry x="5" y="19" width="86" height="14" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-72" value="&lt;font style=&quot;font-size: 11px;&quot;&gt;relu&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E7E8C3;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="T58t_aunDJeNxnw9ZxXW-25" vertex="1">
          <mxGeometry x="5" y="51" width="86" height="14" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-73" value="&lt;span style=&quot;font-size: 11px;&quot;&gt;1x1 conv2d&lt;/span&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#94F7B5;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="T58t_aunDJeNxnw9ZxXW-25" vertex="1">
          <mxGeometry x="5" y="67" width="86" height="14" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-74" value="&lt;span style=&quot;font-size: 11px;&quot;&gt;1x1 conv2d&lt;/span&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#94F7B5;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;" parent="T58t_aunDJeNxnw9ZxXW-25" vertex="1">
          <mxGeometry x="5" y="83" width="86" height="14" as="geometry" />
        </mxCell>
        <mxCell id="vccc8psbofyykT3IaAuy-75" value="&lt;b&gt;...&lt;/b&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;rotation=90;" parent="T58t_aunDJeNxnw9ZxXW-25" vertex="1">
          <mxGeometry x="39" y="95" width="20" height="20" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-27" value="" style="triangle;whiteSpace=wrap;html=1;rotation=-90;strokeColor=none;gradientColor=#737373;gradientDirection=east;" parent="T58t_aunDJeNxnw9ZxXW-25" vertex="1">
          <mxGeometry x="39.38" y="-58.12" width="19.75" height="96.5" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-26" value="" style="shape=image;verticalLabelPosition=bottom;labelBackgroundColor=default;verticalAlign=top;aspect=fixed;imageAspect=0;image=https://cdn-icons-png.flaticon.com/256/9716/9716590.png;" parent="1" vertex="1">
          <mxGeometry x="53" y="115" width="22" height="22" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-31" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.polygon;polyCoords=[[0.06,0],[0.94,0],[1,0.1],[1,0.91],[0.94,1],[0.05,1],[0,0.91],[0,0.1]];polyline=0;fillColor=none;strokeWidth=0.6;dashed=1;" parent="1" vertex="1">
          <mxGeometry x="559.16" y="100.25" width="210.84" height="170" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-32" value="" style="endArrow=classic;html=1;rounded=0;strokeWidth=0.6;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="337" y="215" as="sourcePoint" />
            <mxPoint x="366" y="203" as="targetPoint" />
            <Array as="points">
              <mxPoint x="343" y="215" />
              <mxPoint x="343" y="203" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-51" value="&lt;font face=&quot;Latin Modern Roman&quot;&gt;&lt;b&gt;Step 3. Knapsack-based Optimization (Sec. IIIC)&lt;/b&gt;&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#f5f5f5;fontColor=#000000;strokeColor=default;strokeWidth=0.6;shadow=1;" parent="1" vertex="1">
          <mxGeometry x="570" y="74" width="190" height="30" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-79" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="184" y="146" width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-53" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#E895BB;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-79" vertex="1">
          <mxGeometry width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-60" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-79" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="3" as="sourcePoint" />
            <mxPoint as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-61" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-79" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="6" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-62" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-79" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="9" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-63" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-79" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="12" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-64" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-79" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="15" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-65" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-79" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="18" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-66" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-79" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="21" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-67" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-79" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="24" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-68" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-79" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="27" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-80" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="192" y="146" width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-81" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#E895BB;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-80" vertex="1">
          <mxGeometry width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-82" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-80" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="3" as="sourcePoint" />
            <mxPoint as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-83" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-80" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="6" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-84" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-80" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="9" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-85" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-80" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="12" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-86" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-80" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="15" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-87" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-80" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="18" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-88" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-80" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="21" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-89" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-80" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="24" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-90" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-80" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="27" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-91" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="188" y="146" width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-55" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#28D4D4;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-91" vertex="1">
          <mxGeometry width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-69" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-91" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-70" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-91" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="3" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-71" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-91" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="6" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-72" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-91" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="9" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-73" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-91" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="12" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-74" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-91" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="15" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-75" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-91" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="18" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-76" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-91" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="21" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-77" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-91" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="24" as="sourcePoint" />
            <mxPoint y="27" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-92" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="196" y="146" width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-93" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#28D4D4;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-92" vertex="1">
          <mxGeometry width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-94" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-92" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-95" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-92" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="3" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-96" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-92" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="6" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-97" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-92" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="9" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-98" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-92" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="12" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-99" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-92" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="15" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-100" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-92" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="18" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-101" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-92" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="21" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-102" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-92" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="24" as="sourcePoint" />
            <mxPoint y="27" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-114" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="184" y="201" width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-115" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#E895BB;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-114" vertex="1">
          <mxGeometry width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-116" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-114" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="3" as="sourcePoint" />
            <mxPoint as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-117" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-114" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="6" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-118" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-114" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="9" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-119" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-114" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="12" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-120" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-114" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="15" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-121" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-114" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="18" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-122" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-114" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="21" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-123" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-114" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="24" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-124" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-114" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="27" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-125" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="192" y="201" width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-126" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#E895BB;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-125" vertex="1">
          <mxGeometry width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-127" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-125" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="3" as="sourcePoint" />
            <mxPoint as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-128" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-125" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="6" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-129" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-125" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="9" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-130" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-125" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="12" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-131" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-125" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="15" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-132" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-125" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="18" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-133" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-125" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="21" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-134" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-125" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="24" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-135" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-125" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="27" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-136" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="188" y="201" width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-137" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#28D4D4;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-136" vertex="1">
          <mxGeometry width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-138" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-136" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-139" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-136" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="3" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-140" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-136" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="6" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-141" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-136" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="9" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-142" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-136" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="12" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-143" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-136" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="15" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-144" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-136" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="18" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-145" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-136" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="21" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-146" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-136" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="24" as="sourcePoint" />
            <mxPoint y="27" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-147" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="196" y="201" width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-148" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#28D4D4;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-147" vertex="1">
          <mxGeometry width="4" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-149" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-147" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-150" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-147" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="3" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-151" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-147" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="6" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-152" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-147" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="9" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-153" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-147" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="12" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-154" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-147" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="15" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-155" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-147" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="18" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-156" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-147" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="21" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-157" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-147" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="4" y="24" as="sourcePoint" />
            <mxPoint y="27" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-158" value="&lt;font style=&quot;font-size: 9px;&quot;&gt;...&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="200" y="146" width="14" height="22" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-159" value="&lt;font style=&quot;font-size: 9px;&quot;&gt;...&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="200" y="201" width="14" height="22" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-179" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="283" y="249" width="54" height="21.25" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-177" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#f5f5f5;fontColor=#333333;strokeColor=#000000;strokeWidth=0.6;" parent="T58t_aunDJeNxnw9ZxXW-179" vertex="1">
          <mxGeometry y="1.6200000000000045" width="54" height="18" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-171" value="" style="rounded=0;whiteSpace=wrap;html=1;strokeWidth=0.4;fillColor=#E895BB;" parent="T58t_aunDJeNxnw9ZxXW-179" vertex="1">
          <mxGeometry x="4" y="3.6200000000000045" width="4.75" height="4.75" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-173" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;exitX=1;exitY=1;exitDx=0;exitDy=0;entryX=0;entryY=0;entryDx=0;entryDy=0;" parent="T58t_aunDJeNxnw9ZxXW-179" source="T58t_aunDJeNxnw9ZxXW-171" target="T58t_aunDJeNxnw9ZxXW-171" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="-37" y="-34.379999999999995" as="sourcePoint" />
            <mxPoint x="8" y="-1.3799999999999955" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-174" value="" style="rounded=0;whiteSpace=wrap;html=1;strokeWidth=0.4;fillColor=#28D4D4;" parent="T58t_aunDJeNxnw9ZxXW-179" vertex="1">
          <mxGeometry x="4" y="12.870000000000005" width="4.75" height="4.75" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-175" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;exitX=1;exitY=0;exitDx=0;exitDy=0;entryX=0;entryY=1;entryDx=0;entryDy=0;" parent="T58t_aunDJeNxnw9ZxXW-179" source="T58t_aunDJeNxnw9ZxXW-174" target="T58t_aunDJeNxnw9ZxXW-174" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="-37" y="-25.129999999999995" as="sourcePoint" />
            <mxPoint x="8" y="7.8700000000000045" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-176" value="Memory Access" style="text;html=1;strokeColor=none;fillColor=none;align=left;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Latin Modern Roman;fontSize=6;" parent="T58t_aunDJeNxnw9ZxXW-179" vertex="1">
          <mxGeometry x="8.75" width="45.25" height="12" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-178" value="CPU Execution" style="text;html=1;strokeColor=none;fillColor=none;align=left;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Latin Modern Roman;fontSize=6;" parent="T58t_aunDJeNxnw9ZxXW-179" vertex="1">
          <mxGeometry x="8.75" y="9.25" width="45.25" height="12" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-181" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="306" y="148" width="24" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-182" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#E895BB;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-181" vertex="1">
          <mxGeometry width="10" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-183" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-181" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="2" as="sourcePoint" />
            <mxPoint as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-184" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-181" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="5" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-185" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-181" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="8" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-186" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-181" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="11" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-187" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-181" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="14" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-188" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-181" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="17" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-189" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-181" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="20" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-190" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-181" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="23" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-191" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-181" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="26" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-193" value="" style="group" parent="T58t_aunDJeNxnw9ZxXW-181" vertex="1" connectable="0">
          <mxGeometry x="10" width="14" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-194" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#28D4D4;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-193" vertex="1">
          <mxGeometry width="10" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-195" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-193" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="2" as="sourcePoint" />
            <mxPoint as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-196" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-193" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="5" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-197" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-193" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="8" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-198" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-193" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="11" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-199" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-193" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="14" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-200" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-193" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="17" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-201" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-193" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="20" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-202" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-193" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="23" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-203" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-193" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="10" y="26" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-192" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;" parent="1" vertex="1">
          <mxGeometry x="297" y="138" width="10.53" height="10" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-204" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="306" y="202" width="24" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-205" value="" style="rounded=0;whiteSpace=wrap;html=1;fillStyle=auto;fillColor=#E895BB;gradientColor=none;strokeColor=default;strokeWidth=0.4;" parent="T58t_aunDJeNxnw9ZxXW-204" vertex="1">
          <mxGeometry width="13" height="27" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-206" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-204" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="3" as="sourcePoint" />
            <mxPoint as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-207" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-204" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="6" as="sourcePoint" />
            <mxPoint y="3" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-208" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-204" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="9" as="sourcePoint" />
            <mxPoint y="6" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-209" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-204" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="12" as="sourcePoint" />
            <mxPoint y="9" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-210" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-204" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="15" as="sourcePoint" />
            <mxPoint y="12" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-211" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-204" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="18" as="sourcePoint" />
            <mxPoint y="15" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-212" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-204" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="21" as="sourcePoint" />
            <mxPoint y="18" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-213" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-204" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="24" as="sourcePoint" />
            <mxPoint y="21" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-214" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.3;" parent="T58t_aunDJeNxnw9ZxXW-204" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13" y="27" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-248" value="&lt;font style=&quot;font-size: 9px;&quot;&gt;...&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="324" y="147" width="14" height="22" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-250" value="" style="endArrow=classic;startArrow=classic;html=1;rounded=0;endSize=1;startSize=1;strokeColor=#6B6B6B;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="306" y="178" as="sourcePoint" />
            <mxPoint x="326" y="178" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-251" value="&lt;p style=&quot;line-height: 40%;&quot;&gt;&lt;font face=&quot;Latin Modern Roman&quot; style=&quot;font-size: 7px;&quot;&gt;Decoupling Granularity&lt;/font&gt;&lt;/p&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontColor=#6B6B6B;" parent="1" vertex="1">
          <mxGeometry x="297.14" y="181.25" width="37.73" height="11.5" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-253" value="" style="endArrow=classic;startArrow=classic;html=1;rounded=0;endSize=1;startSize=1;strokeColor=#6B6B6B;entryX=0.907;entryY=0.787;entryDx=0;entryDy=0;entryPerimeter=0;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="306" y="231.75" as="sourcePoint" />
            <mxPoint x="332" y="231.79000000000002" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-254" value="&lt;p style=&quot;line-height: 40%;&quot;&gt;&lt;font face=&quot;Latin Modern Roman&quot; style=&quot;font-size: 7px;&quot;&gt;Decoupling Granularity&lt;/font&gt;&lt;/p&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontColor=#6B6B6B;" parent="1" vertex="1">
          <mxGeometry x="300.27" y="234.5" width="37.73" height="11.5" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-256" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;" parent="1" vertex="1">
          <mxGeometry x="302" y="143" width="10.53" height="10" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-257" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;" parent="1" vertex="1">
          <mxGeometry x="296" y="192" width="10.53" height="10" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-258" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;" parent="1" vertex="1">
          <mxGeometry x="301" y="197" width="10.53" height="10" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-259" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="360" y="105" width="61" height="157.93000000000006" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-33" value="DAE-enabled CNN model" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Latin Modern Roman;fontSize=9;fontStyle=0" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry y="-1" width="61" height="46" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-34" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#f5f5f5;dashed=1;strokeWidth=0.6;fontColor=#333333;strokeColor=#666666;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="6" y="57.93000000000001" width="54" height="97" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-35" value="&lt;font style=&quot;font-size: 6px;&quot;&gt;relu&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E7E8C3;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;fontSize=6;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="9" y="102.93" width="48" height="9" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-36" value="&lt;span style=&quot;font-size: 6px;&quot;&gt;1x1 conv2d&lt;/span&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#94F7B5;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;fontSize=6;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="9" y="115.93" width="48" height="9" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-37" value="&lt;span style=&quot;font-size: 6px;&quot;&gt;1x1 conv2d&lt;/span&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#94F7B5;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;fontSize=6;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="9" y="129.93" width="48" height="9" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-38" value="" style="group" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1" connectable="0">
          <mxGeometry x="6" y="72.93" width="51" height="12" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-39" value="&lt;font style=&quot;font-size: 6px;&quot;&gt;3x3 dw-conv2d&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E8B3E4;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;fontSize=6;" parent="T58t_aunDJeNxnw9ZxXW-38" vertex="1">
          <mxGeometry x="3" y="3" width="48" height="9" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-40" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;strokeWidth=0.5;" parent="T58t_aunDJeNxnw9ZxXW-38" vertex="1">
          <mxGeometry width="6.32" height="6" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-41" value="" style="group" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1" connectable="0">
          <mxGeometry x="6" y="85.93" width="51" height="12" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-42" value="&lt;font style=&quot;font-size: 6px;&quot;&gt;3x3 dw-conv2d&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E8B3E4;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;fontSize=6;" parent="T58t_aunDJeNxnw9ZxXW-41" vertex="1">
          <mxGeometry x="3" y="3" width="48" height="9" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-43" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;strokeWidth=0.5;" parent="T58t_aunDJeNxnw9ZxXW-41" vertex="1">
          <mxGeometry width="6.32" height="6" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-44" value="&lt;b&gt;...&lt;/b&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;rotation=90;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="25" y="56.93000000000001" width="20" height="20" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-45" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;strokeWidth=0.5;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="6" y="112.93" width="6.32" height="6" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-46" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;strokeWidth=0.5;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="6" y="126.93" width="6.32" height="6" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-47" value="&lt;b&gt;...&lt;/b&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;rotation=90;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="25" y="137.93000000000006" width="20" height="20" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-48" value="" style="shape=image;verticalLabelPosition=bottom;labelBackgroundColor=default;verticalAlign=top;aspect=fixed;imageAspect=0;image=https://cdn-icons-png.flaticon.com/256/9716/9716590.png;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="25" y="34.93000000000001" width="15" height="15" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-49" value="" style="triangle;whiteSpace=wrap;html=1;rotation=-90;strokeColor=none;gradientColor=#737373;gradientDirection=east;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="30.44999999999999" y="28.44999999999999" width="6.27" height="50.88" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-50" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;strokeWidth=0.5;" parent="T58t_aunDJeNxnw9ZxXW-259" vertex="1">
          <mxGeometry x="22" y="33.93" width="8.5" height="8.07" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-271" value="" style="endArrow=classic;html=1;rounded=0;fontSize=1;strokeWidth=0.6;entryX=0.001;entryY=0.971;entryDx=0;entryDy=0;endSize=2;entryPerimeter=0;" parent="1" target="T58t_aunDJeNxnw9ZxXW-262" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="418" y="185" as="sourcePoint" />
            <mxPoint x="470" y="160" as="targetPoint" />
            <Array as="points">
              <mxPoint x="424" y="185" />
              <mxPoint x="424" y="147" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-272" value="" style="endArrow=classic;html=1;rounded=0;fontSize=1;strokeWidth=0.6;endSize=2;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="417" y="198" as="sourcePoint" />
            <mxPoint x="442" y="154" as="targetPoint" />
            <Array as="points">
              <mxPoint x="427" y="198" />
              <mxPoint x="427" y="154" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-280" value="" style="endArrow=classic;html=1;rounded=0;fontSize=1;strokeWidth=0.6;endSize=2;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="417" y="213" as="sourcePoint" />
            <mxPoint x="443" y="160" as="targetPoint" />
            <Array as="points">
              <mxPoint x="430" y="213" />
              <mxPoint x="430" y="160" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-281" value="" style="endArrow=classic;html=1;rounded=0;fontSize=1;strokeWidth=0.6;endSize=2;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="417" y="225" as="sourcePoint" />
            <mxPoint x="442" y="166" as="targetPoint" />
            <Array as="points">
              <mxPoint x="433" y="225" />
              <mxPoint x="433" y="166" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-282" value="" style="endArrow=classic;html=1;rounded=0;fontSize=1;strokeWidth=0.6;endSize=2;" parent="1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="417" y="240" as="sourcePoint" />
            <mxPoint x="442" y="172" as="targetPoint" />
            <Array as="points">
              <mxPoint x="437" y="240" />
              <mxPoint x="437" y="172" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-320" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="490" y="207" width="50" height="52.72999999999999" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-319" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#f5f5f5;fontColor=#333333;strokeColor=#000000;strokeWidth=0.6;" parent="T58t_aunDJeNxnw9ZxXW-320" vertex="1">
          <mxGeometry x="4" width="46" height="43" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-289" value="" style="group;fontFamily=Helvetica;fontSize=4;" parent="T58t_aunDJeNxnw9ZxXW-320" vertex="1" connectable="0">
          <mxGeometry y="1" width="49.85" height="51.72999999999999" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-290" value="" style="endArrow=classic;html=1;rounded=0;fontFamily=Helvetica;fontSize=11;strokeWidth=0.6;endSize=2;" parent="T58t_aunDJeNxnw9ZxXW-289" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13.721299969484285" y="32.17112299465241" as="sourcePoint" />
            <mxPoint x="47.94848947207811" y="32.17112299465241" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-291" value="" style="endArrow=classic;html=1;rounded=0;fontFamily=Helvetica;fontSize=11;strokeWidth=0.6;startSize=2;endSize=2;" parent="T58t_aunDJeNxnw9ZxXW-289" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="13.721299969484285" y="32.17112299465241" as="sourcePoint" />
            <mxPoint x="13.69087580103753" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-292" value="&lt;p style=&quot;line-height: 80%; font-size: 7px;&quot;&gt;&lt;font style=&quot;font-size: 7px;&quot;&gt;Energy&lt;/font&gt;&lt;/p&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Latin Modern Roman;fontSize=7;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="14.099101597160605" y="33.72941176470588" width="32.41134649511979" height="6.08235294117647" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-293" value="&lt;p style=&quot;line-height: 80%; font-size: 7px;&quot;&gt;&lt;font style=&quot;font-size: 7px;&quot;&gt;Latency&lt;/font&gt;&lt;/p&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;rotation=-90;fontFamily=Latin Modern Roman;fontSize=7;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="-5.483916880958109" y="12.246641711229941" width="30.42416844675007" height="12.064171122994649" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-294" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="27.062297833384182" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-295" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="30.865318889227947" y="4.021390374331551" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-296" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="34.66833994507169" y="8.042780748663102" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-297" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fillColor=#99FFAD;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="15.653234665852908" y="6.498566844919796" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-298" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="28.2032041501373" y="6.498566844919796" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-299" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="25.601937747940177" y="4.1822459893048265" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-300" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="32.325678974671945" y="9.747850267379706" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-301" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="38.41051266402195" y="9.747850267379683" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-302" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fillColor=#99FFAD;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="17.995895636252666" y="13.60838502673798" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-303" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fillColor=#99FFAD;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="22.93982300884955" y="19.17398930481284" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-304" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fillColor=#99FFAD;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="28.203204150137314" y="22.584128342246" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-305" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fillColor=#99FFAD;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="34.66833994507169" y="24.73959358288771" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-306" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="38.47136100091546" y="12.064171122994649" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-307" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="36.12870003051571" y="13.769240641711253" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-308" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="41.107721829892334" y="13.769240641711232" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-309" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="24.461031431187052" y="10.35910160427807" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-310" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="28.203204150137314" y="12.064171122994649" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-311" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="28.2032041501373" y="15.924705882352947" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-312" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="31.945376869087575" y="17.629775401069526" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-313" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="36.539426304546815" y="17.62977540106951" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-314" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="40.2815990234971" y="19.33484491978609" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-315" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="21.73806835520292" y="4.021390374331551" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-316" value="" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fontFamily=Helvetica;fontSize=11;" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="22.118370460787297" y="8.84705882352941" width="4.203945241919326" height="4.203945241919326" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-321" value="2B" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fillColor=#000000;fontColor=#FFFFFF;fontFamily=Latin Modern Roman;fontSize=10;fontStyle=1" parent="T58t_aunDJeNxnw9ZxXW-289" vertex="1">
          <mxGeometry x="-5.480000000000018" y="33.72999999999999" width="18" height="18" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-322" value="" style="endArrow=classic;html=1;rounded=0;exitX=0.5;exitY=1;exitDx=0;exitDy=0;strokeColor=#3D3D3D;" parent="1" source="T58t_aunDJeNxnw9ZxXW-287" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="380" y="200" as="sourcePoint" />
            <mxPoint x="494" y="227" as="targetPoint" />
            <Array as="points">
              <mxPoint x="448" y="227" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-323" value="&lt;p style=&quot;line-height: 40%;&quot;&gt;&lt;font face=&quot;Latin Modern Roman&quot; style=&quot;font-size: 7px;&quot;&gt;Per Layer Pareto Curve&lt;/font&gt;&lt;/p&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontColor=#6B6B6B;" parent="1" vertex="1">
          <mxGeometry x="448" y="205" width="41" height="11.5" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-324" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="439" y="113" width="135" height="86" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-260" value="" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#f5f5f5;fontColor=#333333;strokeColor=#000000;strokeWidth=0.6;arcSize=9;" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry x="3" width="105" height="80.07" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-262" value="&lt;font style=&quot;font-size: 8px;&quot;&gt;foreach &lt;font style=&quot;font-size: 8px;&quot; color=&quot;#ff0000&quot;&gt;&lt;b style=&quot;font-size: 8px;&quot;&gt;DAE granularity&lt;/b&gt;&lt;/font&gt;&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=left;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Consolas;fontSize=8;" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry x="3" y="24.5" width="108" height="10" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-263" value="&lt;font style=&quot;font-size: 8px;&quot;&gt;foreach&lt;font style=&quot;font-size: 8px;&quot; color=&quot;#ff0000&quot;&gt;&lt;b style=&quot;font-size: 8px;&quot;&gt;&lt;br style=&quot;font-size: 8px;&quot;&gt;&lt;/b&gt;&lt;/font&gt;&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=left;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Consolas;fontSize=8;" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry x="10" y="36" width="95" height="10" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-265" value="&lt;font style=&quot;font-size: 8px;&quot;&gt;foreach&lt;font style=&quot;font-size: 8px;&quot; color=&quot;#ff0000&quot;&gt;&lt;b style=&quot;font-size: 8px;&quot;&gt;&lt;br style=&quot;font-size: 8px;&quot;&gt;&lt;/b&gt;&lt;/font&gt;&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=left;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Consolas;fontSize=8;" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry x="20" y="47" width="95" height="10" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-266" value="&lt;b style=&quot;border-color: var(--border-color); font-family: Consolas; font-size: 7px; text-align: left;&quot;&gt;&lt;font style=&quot;border-color: var(--border-color); font-size: 7px;&quot; color=&quot;#ff0000&quot;&gt;$$F_{\texttt{HSE}}$$&lt;/font&gt;&lt;/b&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontSize=7;" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry x="26" y="34.5" width="60" height="12.5" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-267" value="&lt;b style=&quot;border-color: var(--border-color); font-family: Consolas; font-size: 8px; text-align: left;&quot;&gt;&lt;font style=&quot;border-color: var(--border-color); font-size: 8px;&quot; color=&quot;#ff0000&quot;&gt;$$\texttt{PPLM}$$&lt;/font&gt;&lt;/b&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontSize=8;" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry x="34.5" y="45.75" width="60" height="12.5" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-269" value="&lt;font style=&quot;font-size: 8px;&quot;&gt;foreach&lt;font style=&quot;font-size: 8px;&quot; color=&quot;#ff0000&quot;&gt;&lt;b style=&quot;font-size: 8px;&quot;&gt;&lt;br style=&quot;font-size: 8px;&quot;&gt;&lt;/b&gt;&lt;/font&gt;&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=left;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Consolas;fontSize=8;" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry x="30" y="57" width="95" height="10" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-270" value="&lt;b style=&quot;border-color: var(--border-color); font-family: Consolas; font-size: 8px; text-align: left;&quot;&gt;&lt;font style=&quot;border-color: var(--border-color); font-size: 8px;&quot; color=&quot;#ff0000&quot;&gt;$$\texttt{PPLN}$$&lt;/font&gt;&lt;/b&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontSize=8;" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry x="44.5" y="55.75" width="60" height="12.5" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-274" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.6;dashed=1;dashPattern=1 1;" parent="T58t_aunDJeNxnw9ZxXW-324" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="6" y="41" as="sourcePoint" />
            <mxPoint x="11" y="41" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-275" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.6;dashed=1;dashPattern=1 1;" parent="T58t_aunDJeNxnw9ZxXW-324" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="6" y="52" as="sourcePoint" />
            <mxPoint x="21" y="52" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-276" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=0.6;dashed=1;dashPattern=1 1;" parent="T58t_aunDJeNxnw9ZxXW-324" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="6" y="62" as="sourcePoint" />
            <mxPoint x="31" y="62" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-286" value="Frequency and DAE granularity DSE per layer" style="shape=loopLimit;whiteSpace=wrap;html=1;size=5;fillColor=#1C1C1C;strokeColor=none;fontSize=8;fontFamily=Latin Modern Roman;fontColor=#FFFFFF;" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry x="3" width="105" height="22" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-287" value="2A" style="ellipse;whiteSpace=wrap;html=1;aspect=fixed;fillColor=#000000;fontColor=#FFFFFF;fontFamily=Latin Modern Roman;fontSize=10;fontStyle=1" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry y="68" width="18" height="18" as="geometry" />
        </mxCell>
        <mxCell id="T58t_aunDJeNxnw9ZxXW-288" value="&lt;font style=&quot;font-size: 8px;&quot;&gt;find (t,E)&lt;font style=&quot;font-size: 8px;&quot;&gt;&lt;span style=&quot;font-size: 8px;&quot;&gt;&lt;br style=&quot;font-size: 8px;&quot;&gt;&lt;/span&gt;&lt;/font&gt;&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=left;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Consolas;fontSize=8;fontColor=#3617FF;fontStyle=1" parent="T58t_aunDJeNxnw9ZxXW-324" vertex="1">
          <mxGeometry x="40" y="67" width="95" height="10" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-20" value="Target QoS constraints" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Latin Modern Roman;fontSize=9;fontStyle=0" vertex="1" parent="1">
          <mxGeometry x="570" y="109" width="56" height="29" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-42" value="Per Layer-Frequency Exploration" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#f5f5f5;fontColor=#000000;strokeColor=#000000;rotation=-90;fontFamily=Latin Modern Roman;verticalAlign=middle;" vertex="1" parent="1">
          <mxGeometry x="556" y="173" width="84" height="47.87" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-43" value="" style="endArrow=classic;html=1;rounded=0;exitX=0.263;exitY=0.997;exitDx=0;exitDy=0;entryX=0.5;entryY=0;entryDx=0;entryDy=0;strokeWidth=0.6;exitPerimeter=0;edgeStyle=orthogonalEdgeStyle;" edge="1" parent="1" target="oelAyTeBvST4LJL2yoes-42">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="540" y="229" as="sourcePoint" />
            <mxPoint x="559" y="229" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-47" value="" style="endArrow=classic;html=1;rounded=0;fontSize=1;strokeWidth=0.6;endSize=2;exitX=0.5;exitY=1;exitDx=0;exitDy=0;entryX=1;entryY=0.5;entryDx=0;entryDy=0;" edge="1" parent="1" source="oelAyTeBvST4LJL2yoes-20" target="oelAyTeBvST4LJL2yoes-42">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="632" y="207" as="sourcePoint" />
            <mxPoint x="659" y="255" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-24" value="DAE+DVFS-enabled CNN model" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;fontFamily=Latin Modern Roman;fontSize=9;fontStyle=0" vertex="1" parent="1">
          <mxGeometry x="640" y="105" width="61" height="46" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-26" value="&lt;font style=&quot;font-size: 6px;&quot;&gt;relu&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E7E8C3;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;fontSize=6;" vertex="1" parent="1">
          <mxGeometry x="649" y="213.93" width="48" height="9" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-27" value="&lt;span style=&quot;font-size: 6px;&quot;&gt;1x1 conv2d&lt;/span&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#94F7B5;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;fontSize=6;" vertex="1" parent="1">
          <mxGeometry x="649" y="226.93" width="48" height="9" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-28" value="&lt;span style=&quot;font-size: 6px;&quot;&gt;1x1 conv2d&lt;/span&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#94F7B5;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;fontSize=6;" vertex="1" parent="1">
          <mxGeometry x="649" y="240.93" width="48" height="9" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-29" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="646" y="183.93" width="51" height="12" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-30" value="&lt;font style=&quot;font-size: 6px;&quot;&gt;3x3 dw-conv2d&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E8B3E4;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;fontSize=6;" vertex="1" parent="oelAyTeBvST4LJL2yoes-29">
          <mxGeometry x="3" y="3" width="48" height="9" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-31" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;strokeWidth=0.5;" vertex="1" parent="oelAyTeBvST4LJL2yoes-29">
          <mxGeometry width="6.32" height="6" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-32" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="646" y="196.93" width="51" height="12" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-33" value="&lt;font style=&quot;font-size: 6px;&quot;&gt;3x3 dw-conv2d&lt;/font&gt;" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#E8B3E4;strokeColor=#000000;perimeterSpacing=1;strokeWidth=0.6;fontFamily=Latin Modern Roman;fontSize=6;" vertex="1" parent="oelAyTeBvST4LJL2yoes-32">
          <mxGeometry x="3" y="3" width="48" height="9" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-34" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;strokeWidth=0.5;" vertex="1" parent="oelAyTeBvST4LJL2yoes-32">
          <mxGeometry width="6.32" height="6" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-35" value="&lt;b&gt;...&lt;/b&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;rotation=90;" vertex="1" parent="1">
          <mxGeometry x="665" y="167.93" width="20" height="20" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-36" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;strokeWidth=0.5;" vertex="1" parent="1">
          <mxGeometry x="646" y="223.93" width="6.32" height="6" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-37" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;strokeWidth=0.5;" vertex="1" parent="1">
          <mxGeometry x="646" y="237.93" width="6.32" height="6" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-38" value="&lt;b&gt;...&lt;/b&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;rotation=90;" vertex="1" parent="1">
          <mxGeometry x="665" y="248.93000000000006" width="20" height="20" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-39" value="" style="shape=image;verticalLabelPosition=bottom;labelBackgroundColor=default;verticalAlign=top;aspect=fixed;imageAspect=0;image=https://cdn-icons-png.flaticon.com/256/9716/9716590.png;" vertex="1" parent="1">
          <mxGeometry x="665" y="145.93" width="15" height="15" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-40" value="" style="triangle;whiteSpace=wrap;html=1;rotation=-90;strokeColor=none;gradientColor=#737373;gradientDirection=east;" vertex="1" parent="1">
          <mxGeometry x="670.45" y="139.45" width="6.27" height="50.88" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-41" value="" style="verticalLabelPosition=bottom;verticalAlign=top;html=1;shape=mxgraph.basic.star;fillColor=#F8FF21;strokeWidth=0.5;" vertex="1" parent="1">
          <mxGeometry x="662" y="144.93" width="8.5" height="8.07" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-52" value="" style="endArrow=classic;html=1;rounded=0;entryX=0.022;entryY=0.491;entryDx=0;entryDy=0;exitX=0.5;exitY=1;exitDx=0;exitDy=0;strokeWidth=0.6;endSize=2;entryPerimeter=0;edgeStyle=orthogonalEdgeStyle;" edge="1" parent="1" source="oelAyTeBvST4LJL2yoes-42" target="oelAyTeBvST4LJL2yoes-30">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="620" y="250" as="sourcePoint" />
            <mxPoint x="670" y="200" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-53" value="" style="endArrow=classic;html=1;rounded=0;entryX=0.019;entryY=0.528;entryDx=0;entryDy=0;exitX=0.5;exitY=1;exitDx=0;exitDy=0;strokeWidth=0.6;endSize=2;entryPerimeter=0;edgeStyle=orthogonalEdgeStyle;" edge="1" parent="1" source="oelAyTeBvST4LJL2yoes-42" target="oelAyTeBvST4LJL2yoes-33">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="620" y="200" as="sourcePoint" />
            <mxPoint x="658" y="201" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-54" value="" style="endArrow=classic;html=1;rounded=0;entryX=0.019;entryY=0.54;entryDx=0;entryDy=0;exitX=0.5;exitY=1;exitDx=0;exitDy=0;strokeWidth=0.6;endSize=2;entryPerimeter=0;edgeStyle=orthogonalEdgeStyle;" edge="1" parent="1" source="oelAyTeBvST4LJL2yoes-42" target="oelAyTeBvST4LJL2yoes-27">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="632" y="207" as="sourcePoint" />
            <mxPoint x="658" y="214" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-55" value="" style="endArrow=classic;html=1;rounded=0;entryX=0.013;entryY=0.548;entryDx=0;entryDy=0;exitX=0.5;exitY=1;exitDx=0;exitDy=0;strokeWidth=0.6;endSize=2;entryPerimeter=0;edgeStyle=orthogonalEdgeStyle;" edge="1" parent="1" source="oelAyTeBvST4LJL2yoes-42" target="oelAyTeBvST4LJL2yoes-28">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="620" y="200" as="sourcePoint" />
            <mxPoint x="658" y="241" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-56" value="STM32 MCU Deployment" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#f5f5f5;fontColor=#000000;strokeColor=#000000;rotation=-90;fontFamily=Latin Modern Roman;verticalAlign=middle;" vertex="1" parent="1">
          <mxGeometry x="701" y="174.06" width="84" height="39.87" as="geometry" />
        </mxCell>
        <mxCell id="oelAyTeBvST4LJL2yoes-57" value="" style="endArrow=classic;html=1;rounded=0;entryX=0.5;entryY=0;entryDx=0;entryDy=0;strokeWidth=0.6;edgeStyle=orthogonalEdgeStyle;" edge="1" parent="1" target="oelAyTeBvST4LJL2yoes-56">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="700" y="217" as="sourcePoint" />
            <mxPoint x="311" y="221" as="targetPoint" />
            <Array as="points">
              <mxPoint x="712" y="217" />
              <mxPoint x="712" y="194" />
            </Array>
          </mxGeometry>
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>


==> sections/01_related.tex <==
\section{Related Work}
\label{sec:related}

\cite{lin2020mcunet} - Tiny Deep Learning on IoT Devices

\cite{lin2022device} - On-device training under 256kb
\cite{sudharsan2021ml} - ML-MCU: A Framework to Train ML Classifiers
on MCU-Based IoT Edge Devices
\cite{banbury2021micronets} - Micronets: Neural network architectures for deploying tinyml applications on commodity microcontrollers

\cite{liberis2021munas} - $\mu$NAS: Constrained neural architecture search for microcontrollers

\cite{jaiswal2023minun} - MinUn: Accurate ML Inference on Microcontrollers

\cite{wang2020fann} - FANN-on-MCU: An open-source toolkit for energy-efficient neural network inference at the edge of the Internet of Things

\begin{itemize}
    \item Can we somehow classify the related literature? (2 paragraphs is fine)
    \\\textbf{DVFS for machine learning workloads}
    Several works have explored the use of dynamic voltage frequency scaling and optimal decoupled access execution strategies for different workloads\EA{\cite{XXX}}. These approaches often consider well-known benchmarks, yet fail to offer decoupling solutions for deep neural networks\EA{\cite{XXX}}.
    \\\textbf{DVFS in MCUs}
    Most DVFS approaches focus on bigger devices (such as GPUs) with multiple cores and rely on inter-core communication for their decoupled access execution implementations \EA{\cite{XXX}} %https://arxiv.org/pdf/1701.05478.pdf
    . Single-core approaches to DVFS have often been overlooked due to the high frequency switching overhead \EA{\cite{XXX}} %https://www.mdpi.com/2076-3417/11/6/2581
    However these approaches often fail to consider optimization of switching techniques with utilization of different clock sources, as well as decoupled access execution techniques that have been fine-tuned according to the workload domain. 
        \item Clearly indicate the key differences and missing points in the existing research. 
    \\To the best our knowledge, there has been no DVFS implementation with decoupled access execution for machine learning workloads on ARM Cortex M MCUs, or any TinyML devices. There has also been no approach where clock parameters and sources have been co-designed to obtain the optimal strategy for DVFS in deep neural networks.
    \\


\end{itemize}

==> tables/acronyms.tex <==
\setlength\extrarowheight{2pt}
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ p{0.2\columnwidth}|p{0.8\columnwidth}}
\Xhline{4\arrayrulewidth}
\cellcolor[HTML]{EFEFEF}{\textbf{Acronym}} & \cellcolor[HTML]{EFEFEF}{\textbf{Short Description}} \\
\Xhline{4\arrayrulewidth}
\textbf{HSI} & \textbf{H}igh \textbf{S}peed \textbf{I}nternal clock. Used as an intermediate 
clock to continue operation when the PLL is off                   \\
\hline
\textbf{HSE} & \textbf{H}igh \textbf{S}peed \textbf{E}xternal clock \\
\hline
\textbf{PLL} & \textbf{P}hase \textbf{L}ocked \textbf{L}oop. Consists of PLLM, PLLN, PLLP, PLLQ parameters used to adjust the input frequency \\
\hline
\textbf{DAE} & \textbf{D}ecoupled \textbf{A}ccess \textbf{E}xecution \\
\hline
\textbf{Granularity N } & Number of buffers (N) to be decoupled \\           
\Xhline{4\arrayrulewidth}                                                    
\end{tabular}}
\caption{Acronym description}
\label{table:acronyms}
\end{table}

==> tables/clock_startup_vco_datasheet.tex <==
\begin{table}[]
\begin{tabular}{llllll}
Symbol                 & Parameter                      & Conditions         & Min & Max & Unit                \\
\multirow{2}{*}{$t_{lock}$} & \multirow{2}{*}{PLL lock time} & VCO freq = 192 MHz & 75  & 200 & \multirow{2}{*}{$\mu$s} \\
                       &                                & VCO freq = 432 MHz & 100 & 300 &                    
\end{tabular}
\label{table:clock_startup_vco_datasheet}
\caption{Clock startup time values depending on VCO - Datasheet reference}
\end{table}

==> tables/current_consumption_datasheet.tex <==
\begin{table}[]
\begin{tabular}{m{1cm}m{2.5cm}m{2cm}m{0.5cm}m{0.5cm}m{0.5cm}}
Symbol                    & Parameter                                                                                & Conditions         & Min  & Max  & Unit                \\
\multirow{2}{*}{$I_{DD(PLL)}$} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}PLL power \\ consumption on VDD\end{tabular}} & VCO freq = 192 MHz & 0.15 & 0.4  & \multirow{2}{*}{mA} \\
                          &                                                                                          & VCO freq = 432 MHz & 0.45 & 0.75 &                    
\end{tabular}
\label{table:current_consumption_vco}
\caption{Current consumption depending on VCO value - Datasheet reference}
\end{table}

==> tables/power_startup.tex <==
\begin{table}[]
\begin{tabular}{|m{1cm}| m{0.75cm}| m{1cm}| m{1cm}| m{1cm}| m{1cm}| m{1cm}|}
\hline
Input Frequency (MHz) & Output Frequency (MHz) & PLLN & PLLM & Power after switching (mW) & Switching time (mus) & Power during switching (mW) \\
\hline
50                    & 216                    & 216  & 25   & 74                         & 64                   & 41                          \\
\hline
50                    & 216                    & 432  & 50   & 74                         & 119                  & 41                          \\
\hline
50                    & 168                    & 168  & 25   & 54                         & 76                   & 41                          \\
\hline
50                    & 168                    & 336  & 50   & 54                         & 115                  & 41       \\
\hline
\end{tabular}
\caption{Power Consumption \& clock startup time for different PLL parameters \EA{Plot this(?), Merge tables, remove redundant data}}
\label{table:power_startup}
\end{table}

==> tables/power_stm32f4.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{p{0.22\columnwidth}|p{0.1\columnwidth}|p{0.1\columnwidth}|p{0.23\columnwidth}|p{0.23\columnwidth}}
\Xhline{4\arrayrulewidth}
\cellcolor[HTML]{EFEFEF}{\textbf{HSE frequency (MHz)}} & \cellcolor[HTML]{EFEFEF}{\textbf{PLLM}} & \cellcolor[HTML]{EFEFEF}{\textbf{PLLN}} & \cellcolor[HTML]{EFEFEF}{\textbf{Output frequency (MHz)}}  & \cellcolor[HTML]{EFEFEF}{\textbf{Power consumption (mW)}} \\
\Xhline{4\arrayrulewidth}
16 & 15 & 187  & 99 & 29 \\
\hline
\cellcolor[HTML]{EFEFEF}{16} & \cellcolor[HTML]{EFEFEF}{8} & \cellcolor[HTML]{EFEFEF}{100}  & \cellcolor[HTML]{EFEFEF}{100} & \cellcolor[HTML]{EFEFEF}{28} \\
\hline
20 & 10 & 100  & 100  & 23 \\
\hline
\cellcolor[HTML]{EFEFEF}{25} & \cellcolor[HTML]{EFEFEF}{25} & \cellcolor[HTML]{EFEFEF}{200}  & \cellcolor[HTML]{EFEFEF}{100} & \cellcolor[HTML]{EFEFEF}{20} \\
\hline
30 & 30 & 200  & 100 & 16 \\
\hline
\cellcolor[HTML]{EFEFEF}{30} & \cellcolor[HTML]{EFEFEF}{15} & \cellcolor[HTML]{EFEFEF}{100}  & \cellcolor[HTML]{EFEFEF}{100} & \cellcolor[HTML]{EFEFEF}{16} \\
\hline
50 & 50 & 200  & 100 & 13 \\
\hline
\cellcolor[HTML]{EFEFEF}{50} & \cellcolor[HTML]{EFEFEF}{25} & \cellcolor[HTML]{EFEFEF}{100} & \cellcolor[HTML]{EFEFEF}{100} & \cellcolor[HTML]{EFEFEF}{11} \\
\Xhline{4\arrayrulewidth}
\end{tabular}}
\caption{Power Consumption Sensitivity Analysis - STM32F4}
\label{table:power_stm32f4}
\end{table}

==> tables/power_stm32f7.tex <==
\begin{table}[b]
\resizebox{\columnwidth}{!}{
\begin{tabular}{p{0.32\columnwidth}|p{0.1\columnwidth}|p{0.1\columnwidth}|p{0.35\columnwidth}}
\Xhline{4\arrayrulewidth}
\rowcolor{gray!25} \textbf{HSE frequency (MHz)} & \textbf{PLLM} & \textbf{PLLN} & \textbf{Power consumption (mW)} \\
\Xhline{4\arrayrulewidth}
16 & 8 & 216 & 123 \\
\hline
\rowcolor{gray!25} 16 & 15   & 405  & 121 \\
\hline
20 & 10   & 216  & 100 \\
\hline
\rowcolor{gray!25} 25 & 25 & 432 & 85 \\
\hline
30 & 30   & 432  & 74 \\
\hline
\rowcolor{gray!25} 30 & 15 & 216 & 72 \\
\hline
50 & 50   & 432  & 52 \\
\hline
\rowcolor{gray!25} \textbf{50} & \textbf{25} & \textbf{216} & \textbf{50} \\
\Xhline{4\arrayrulewidth}
\end{tabular}}
\caption{Power Consumption Sensitivity Analysis for system clock at at 216MHz of STM32F7 for different \texttt{HSE} and \texttt{PLL} configurations.}
\label{table:power_stm32f7}
\end{table}
